Parameterized Algebraic Protocols

We propose algebraic protocols that enable the definition of protocol templates and session types analogous to the definition of domain-specific types with algebraic datatypes. Parameterized algebraic protocols subsume all regular as well as most context-free and nested session types and, at the same time, replace the expensive superlinear algorithms for type checking by a nominal check that runs in linear time. Algebraic protocols in combination with polymorphism increase expressiveness and modularity by facilitating new ways of parameterizing and composing session types.

==> action.tex <==
\section{Action!}

\input{example-sendtree}
\input{example-streaming}
\input{example-arithserver}
\input{example-repeater}
\input{example-secureme}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> algorithmic.tex <==
\section{Algorithmic rules}
\label{sec:alg}

% \subsection{Algorithmic type formation}
% \input{fig-alg-type-formation}

\subsection{Expressions}
% \input{fig-type-constants}

% \begin{align*}
%   \termc e &::= \termc x
%              \mid \termc c
%              \mid \abse xTe
%              \mid \tabse x\kind e
%              \mid \appe ee
%              \mid \paire ee
%              \mid \lete xyee\\
%            & \mid \inje \ell e
%              \mid \casee e {\{\ell \rightarrow e_\ell\}_{\ell \in L}}
%              \mid \casee e {\{\constr\ \overline{x} \rightarrow e_\constr\}_{\constr \in P}}
%              \mid \tappe eT
%              \mid \newe T
%              \mid \ESelect e
% \end{align*}

\todo{\exps{match} ?\quad records: $\termc {\{\ell = e_\ell\}_{\ell
      \in L}}$ ? or just pairs? \quad more ?}
\pt{records and variants should be subsumed by data protocols.}
% \subsection{Algorithmic typing}
% \input{fig-alg-typing}

\pt{Need to check rules from E-Ctor to end because the rules for
  protocol definition changed.}
\pt{I'm wondering if we can create a E-case2 rule similar to the
  E-select rule. I.e., the variant would deal with just one
  constructor and have a default case for the remaining ones.}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> attic.tex <==

\begin{lstlisting}
compose : (X, C) -> (C -> (Y, C')) -> ((X, Y), C') -- aka (#>)
compose xc f = let (x, c) = xc in
                          let (y, c) = f c in
                          ((x,y), c)
fmap : (X, C) -> (X -> Y) -> (Y, C)                    -- Haskell (<&>)
fmap (x, c) f = (f x, c)

ILeaf_P c -> receive [Int, s] c <&> ILeaf
INode_P c -> recvITree [?ITree_P.s] c #> recvITree [s] <&> uncurry INode
\end{lstlisting}

Or better yet:
\begin{lstlisting}
(<*>) : (C1 -> (A -> B, C2)) -> (C2 -> (A, C3)) -> (C1 -> (B, C3))
fab <*> fa = \c1 ->  let (f, c2) = fab c1 in
                               let (a, c3) = fa c2 in
                               (f a, c3)

pure : X -> (C -> (X, C))
pure x c = (x, c)

ILeaf_P c  -> c |> (pure ILeaf <*> receive [Int, s])
INode_P c -> c |> (pure INode <*> recvITree [?ITree_P.s]) <*> recvITree [s]

\end{lstlisting}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> cfst-vs-algst.tex <==
\section{Embedding context-free session types}
\label{sec:cfst-vs-algst}

% PT: this should be integrated in the related work paragraph to avoid repetition

% In this section we informally compare the metatheory
% of algebraic session types with that of context-free session types. Although
% these theories are closely related expressivity-wise, the abstraction mechanisms
% underlying algebraic and context-free session types are quite different:
% algebraic session types parameterize over behavior, whereas context-free session
% types abstract over the exchanged messages. Consider the example of the
% \lstinline{Stream} protocol presented in~\cref*{sec:param-prot}:

% \begin{lstlisting}
%     protocol Stream (a:P) = Next a (Stream a)
% \end{lstlisting}

% The direction of the communication is not settled until the parameter is
% instantiated and the protocol is materialized: a stream of integer values is
% governed by type $\TOut{\mathsf{Stream\,Int}}{\TEndT}$, while a process
% that receives integers \emph{ad aeternum} may be typed by
% $\TOut{\mathsf{Stream\,-Int}}{\TEndT}$. If we were to define a context-free
% counterpart for \lstinline|Stream|, we could think of types
% $\forall \alpha\colon\kindm. \mu x\colon \kinds. !\alpha; x$ or
% $\forall \alpha\colon\kindm. \mu x\colon \kinds. ?\alpha; x$ but both commit to
% a concrete direction. Protocol \lstinline{Stream} abstracts the direction
% through parameter \lstinline{a}. One could argue that these could be achieve
% with higher-order types, in the lines of
% \citet{DBLP:journals/corr/abs-2203-12877}, but, to the best of our knowledge,
% handling fully polymorphic sessions (read, assign kind $\kinds$ to polymorphic
% types) is still an open problem. For these reasons, we claim that algebraic
% session types are more expressive than context-free session types.

This section presents an informal investigation of two questions that relate \algst and
context-free session types (CFST
\cite{DBLP:journals/corr/abs-2106-06658}): can we map any \algst
program into an equivalent CFST program? And: can we map any CFST program to an
equivalent \algst program?

This investigation is necessarily informal because the features of
\algst and CFST do not line up. \algst is a minimalist mostly linear
version of System~F with products, sessions, and algebraic
protocols. CFST is also based on System~F, but has a richer kind
structure that enables unrestricted as well as linear features,
variant and record types, and the full slate of context-free session
primitives.

To enable a meaningful comparison,  we focus on the linear fragment of
CFST~\cite{DBLP:journals/corr/abs-2106-06658}
using the notation of \citet{DBLP:journals/corr/abs-2203-12877},
restricted to pairs and ignoring De Bruijn indices.
In \algst, we only consider types that are not polymorphic in
protocols because CFST has no equivalent. We add linear algebraic
datatypes to cope with variant types in CFST.

% We decided to 
% present the theory of algebraic session types in a simplified form: all types are linear, 
% we do not have records and we omitted the definition of $\datak$type definitions in 
% the formalization of our system (despite the obvious similarities with $\protocolk$ definitions). 
% For that reason, this comparison should 
% be considered in a loose, rather than in a strict, sense. In the context-free side, we 
% consider pairs instead of records as well.

% and ignore De Bruijn 
%indices (as used by Costa et al.~\cite{DBLP:journals/corr/abs-2203-12877}) because they would 
%unnecessarily burden the analysis.

%\input{fig-algst-vs-cfst}

\paragraph{Non-parameterized algebraic sessions into (linear) context-free sessions} 
The translation from 
algebraic session types that do not parameterize over protocol types
(AlgST${}_0$) to context-free session types 
(CFST)  is  given by $\algsttocfst{\typec T}$, which is defined on
types in normal form, only:
\begin{mathpar}
    \algsttocfst{\TUnit} = \syntax{unit} \quad
    \algsttocfst{\TFun[]TU} = \algsttocfst {\typec{T}} \rightarrow \algsttocfst {\typec{U}} \quad
    \algsttocfst{\TPair TU} = \algsttocfst {\typec{T}} \times \algsttocfst {\typec{U}}\quad
    \algsttocfst{\TForall{\alpha}{\kindt} T} = \forall \alpha:\kindtl. \algsttocfst {\typec{T}}\\
	\algsttocfst{\typec{\alpha}} = \alpha\qquad
	%% sessions
	\algsttocfst{\TIn{T}{U}}= ?\algsttocfst{\typec{T}}; \algsttocfst{\typec U} \qquad
	\algsttocfst{\TOut{T}{U}}= !\algsttocfst{\typec T}; \algsttocfst{\typec U} \qquad 
	\algsttocfst{\TEndT} = \syntax{skip} \qquad 
	\algsttocfst{\TEndW} = \syntax{skip}\\
	\algsttocfst{\TIn{\TPApp{P}{\overline U}}{S}}= P_U; \algsttocfst{\typec S} 
	\text{ where } 
	P_U \doteq \&\{ C_i\colon
	\algsttocfst{\TFIn {\overline{T_i[\overline U/\overline\alpha]}}{\TEndT}} \}_{i\in I}
	\text{ for }
\protocolk\ \typec{\proto\ \overline{\alpha}}~\blk{=}~\typec{\{{\termc{\constr_i}\ \overline{T_i}}\}_{i\in I} } \\
	\algsttocfst{\TOut{\TPApp{P}{\overline U}}{S}}= P_U; \algsttocfst{\typec S} 
	\text{ where } 
	%% \algsttocfst{\polarizedparam{-}{T}} = \syntax{dual}\, \algsttocfst{\typec T} \\
	P_U \doteq \oplus\{ C_i\colon
        \algsttocfst{\TFOut {\overline{T_i[\overline U/\overline\alpha]}}{\TEndT}} \}_{i\in I}
        \text{ for }
	\protocolk\ \typec{\proto\ \overline{\alpha}}~\blk{=}~\typec{\{{\termc{\constr_i}\ \overline{T_i}}\}_{i\in I} }
    \end{mathpar}

Functional types and 
message exchanges are naturally mapped onto their counterparts. The end of a session is mapped 
to $\syntax{skip}$, whereas algebraic protocols are translated to
type names defined as internal choices or branches, depending on whether they appear 
in sending or receiving positions. The choice labels coincide with the protocol
constructors. 

We claim that if $\isEquiv{T}{U}$, then $\algsttocfst{\typec T}\simeq\algsttocfst{\typec U}$.

\input{fig-cfst-vs-algst}

\paragraph{Linear context-free sessions embedded into algebraic sessions} 
In this direction, we omit polymorphism to obtain a lighter, more
perspicuous notation. Our comparative approach scales to the
polymorphic setting, but at the price of high notational overhead as
pointed out in \cref{sec:appendix-cfst-algst}. 

The translation of the \emph{linear} and \emph{monomorphic} fragment of CFST 
to AlgST is split between the functional and the session typed fragments,
which are mutually defined and presented in~\cref{fig:cfst-vs-algst-f}. The translation of a
context-free session type $T$ to the algebraic setting is given by $\cfsttoalgst T$. 
The functional operators have natural counterparts in the algebraic side.
When translated to the isorecursive setting, functional recursive types are represented 
by a datatype enclosed with an explicit unfold. Variant types are mapped to datatypes whose 
constructors are the respective labels. Session types are materialized by protocol definitions:
each session type originates a protocol emerging from the conversion of a sequential composition of 
types into a sequence of (algebraic) types with kind $\kindp$. 
This conversion is governed by function $\cfsttoprot{\cdot}$ that maps $\syntax{skip}$
to the empty sequence and uses polarities to enforce the direction of communication.
In the session typed fragment, recursive types and choices are represented by protocol definitions.
Type names are considered generative and we relax \algst to admit 
overloaded constructor names that can be reused across protocol definitions.

%\input{table-iso-cfst-to-algst}

It remains to define suitable adapters in the places where CFST relies
on type equivalence of equirecursive types. To this end we generate
isomorphisms as witnesses of equivalence proofs using the rule system
proposed by \citet{DBLP:journals/corr/abs-2203-12877}. 
The tricky part of constructing such an isomorphism is its extension
into session types. 
For simplicity, we consider just one side of the isomorphism
$\mathsf{iso} : \cfsttoalgst{T} \rightarrow \cfsttoalgst{U}$ 
where $T \simeq U$ as session types:
\begin{lstlisting}
iso t = let (u, u') = new [|U|] in fork $ delta t u' |> u
\end{lstlisting} %$
This definition relies on a process $\delta : \cfsttoalgst{T} \to
\TDual{\cfsttoalgst{U}} \to \TUnit$ that consumes two (dual) channel
ends and implements a forwarder that compensates for the differences
between $T$ and $U$. The witness processes $\delta$ are 
defined for each pair of equivalent session types, according 
to the rules. We sketch some witness 
processes in \cref{sec:appendix-cfst-algst} and provide a more detailed analysis of the isomorphism. 

In general, $\delta$ inserts the explicit unfolds imposed by the translation to the isorecursive setting.
We showcase our approach for the equivalence $Y \simeq U$ where type $Y$ is defined by $T$, $Y \doteq T$.
The definition of $\delta$ follows the equivalence rule of \citet{DBLP:journals/corr/abs-2203-12877}
and shown below.
%
A witness process $\delta$ for the embedding $\mathsf{iso} : \cfsttoalgst{Y} \rightarrow \cfsttoalgst{U}$  
builds on a process $\delta_1$ witnessing $T \simeq U$ and is defined by:

\begin{minipage}{0.6\textwidth}
\begin{lstlisting}
delta y u = match u with {
   XU u -> let y = select XY y in 
           let t = select UnfoldY y in
           delta1 t u }
\end{lstlisting}
\end{minipage}
\begin{minipage}{0.4\textwidth}
	$$\inferrule{Y\doteq T \\ T\,\mathsf{contr}\\\isodecl{\delta_1} T \simeq U}{\isodecl{\delta} Y \simeq U}$$
\end{minipage}

As a result of the definition of $\cfsttoalgst{Y\colon \mathsf{S^{lin}}}$, 
process $\delta$ \lstinline|match|es with $X_U$ on channel $u$ and \lstinline|select|s $X_Y$ on channel $y$, as prescribed by the
protocol definitions resulting from $\cfsttoalgst{\syntax{Y}}$ (see~\cref{fig:cfst-vs-algst-f}). Then, 
 \lstinline|select|s the explicit $\termc{\mathsf{Unfold}_Y}$ introduced by $\cfsttoprot{Y}$ and 
uses $\delta_1$ to consume the leftovers at $t$ and $u$.

%Other cases and a more thorough analysis can be found in \cref{sec:appendix-cfst-algst}. 
For the
other direction of the isomorphism, we could follow a similar approach for defining 
$\mathsf{iso}^{-1} : \cfsttoalgst{U} \rightarrow \cfsttoalgst{T}$ 
and then prove that $\mathsf{iso}$ and $\mathsf{iso}^{-1}$ compose giving the identity.
To extend the translation to the polymorphic fragment, we would need to consider a 
\emph{reader monad} to store a map from type variables to the auxiliary processes
that consume the respective channel ends.
 
% In the case of $!T; V \simeq !U;W$, we are provided not only with a witness $\delta_1$ to consume the remainder
% of channels $v$ and $w$, but also with a function $\theta \colon \cfsttoalgst{T} \rightarrow \cfsttoalgst{U}$
% that witnesses the isomorphism resulting from $T\simeq U$. The functions witnessing the isomorphism 
% between types in the functional fragment are presented in~\cref{tab:iso-cfst-to-algst-f}.
% Given $\delta_1$ and $\theta$, process $\delta$ \lstinline|receive|s $u$ on channel $w$, 
% transforms $u$ with $\theta^{-1}$ and sends the result through channel $v$. Process
% $\delta_1$ consumes the remainder of $v$ and $w$.

% To witness the isomorphism corresponding to $!T; V \simeq !U$ where $V$ is a 
% terminated session (see \citet{DBLP:journals/corr/abs-2203-12877} for further details), we are given
% a process $\sigma$ that consumes the explicit unfolds resulting from the isorecursive interpretation of $V$. The 
% \emph{consumer} processes $\sigma$ for terminated sessions are presented in \cref{tab:iso-is-terminated}.

% The other cases in \cref{tab:iso-cfst-to-algst-f,tab:iso-witness-sessions,tab:iso-is-terminated} follow
% a similar reasoning. The omitted cases for monomorphic types also fit the same approach. For the polymorphic 
% fragment, we would need to consider a \emph{reader monad} where one could store a map from type
% variables to the processes that consume the corresponding channels or transform the 
% corresponding values, depending on whether the type variables are of kind $\kinds$ or not. 
% In the axiom for polymorphic (non-session typed) variables $n\simeq n$, for instance,
% %\begin{mathpar}
% %\axiom{}{\isodecl{\theta} n}\simeq n}
% %\end{mathpar}
% we could think of $\theta$ as the identity function, but we wouldn't know which type to 
% assign to the bound variable: $\theta = \abse{x}{?}{x}$. Whereas to consume two channels 
% typed with a polymorphic session-typed variable, we would need to know how to consume both
% endpoints.
% %
% %$\inferrule{\isodecl{\sigma} T\checkmark}{\isodecl{\delta} n;T \simeq n}$
% %
% Processes to consume or transform values typed with polymorphic variables would need to 
% be provided to $\delta$. For the translation of types in the polymorphic fragment, we would need to collect the free
% variables occurrig in the type and use a parametrized $\datak$ or $\protocolk$ definition:
% \begin{mathpar}
% \cfsttoalgst{X\colon \kappa} = \typec{X\ \overline{\alpha}}
% 	\text{ for } X \doteq T \text{ and } \kappa \neq \mathsf{S^{lin}}
% 	\text{ where } \datak\ \typec{X\ \overline{\alpha}}~\blk{=}~\typec{\termc{\mathsf{Unfold}_X}\ \cfsttoalgst{T}} \text{ and }\FVL{T} = \overline\alpha
% 	\and 
% 	\cfsttoprot{X\colon \mathsf{S^{lin}}} = \typec{X\ \overline{\alpha}}
% 	\text{ for } X \doteq T
% 	\text{ where }
% 	\protocolk\ \typec{X\ \overline{\alpha}}~\blk{=}~\typec{\termc{\mathsf{Unfold}_X}\ \cfsttoprot{T}} 
% 	\text{ and }\FVL{T} = \overline\alpha
% \end{mathpar}
% %
% Although we believe that polymorphic types
% do not pose any problem to this analysis, we decided to keep the notation simple and
% focus on the monomorphic fragment.

% In this analysis we only provided witnesses for the "isomorphism" in one direction.
% For the other direction, we could follow a similar approach and then prove that 
% they are inverses of each other.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> fig-algst-vs-cfst.tex <==
\begin{figure}[t!]
  \declrel{AlgST${}_0$ to CFST: Translation of algebraic to context-free session types}{$\algsttocfst{\typec T}=T$}
 
    \begin{mathpar}
    \algsttocfst{\TUnit} = \syntax{unit} \quad
    \algsttocfst{\TFun[]TU} = \algsttocfst {\typec{T}} \rightarrow \algsttocfst {\typec{U}} \quad
    \algsttocfst{\TPair TU} = \algsttocfst {\typec{T}} \times \algsttocfst {\typec{U}}\quad
    \algsttocfst{\TForall{\alpha}{\kindt} T} = \forall \alpha. \algsttocfst {\typec{T}}\quad
	\algsttocfst{\typec{\alpha}} = \alpha\\
	%% sessions
	\algsttocfst{\TIn{T}{U}}= ?\algsttocfst{\typec{T}}; \algsttocfst{\typec U} \quad 
	\algsttocfst{\TOut{T}{U}}= !\algsttocfst{\typec T}; \algsttocfst{\typec U} \quad 
	\algsttocfst{\TEndT} = \syntax{skip} \quad 
	\algsttocfst{\TEndW} = \syntax{skip}\quad
	\algsttocfst{\polarizedparam{-}{T}} = \syntax{dual}\, \algsttocfst{\typec T} \\ 
	\algsttocfst{\TPApp{P}{\overline T}} = \oplus\{ C_i\colon \algsttocfst{\tosession{T_i^1}{\TEndT}} ; \ldots;\algsttocfst{\tosession{T_i^{n_i}}{\TEndT}}\}_{i\in I}  \text{ when }
	\protocolk\ \typec{\proto\ \overline{\alpha}}~\blk{=}~\typec{\{{\termc{\constr_i}\ T_i^1\ldots T_i^{n_i}}\}_{i\in I} }
    \end{mathpar}
\caption{Translation of algebraic session types to context-free session types}
\label{fig:algst-to-cfst}
\end{figure}


==> fig-ctx.tex <==
\begin{figure}
\declrel{Context formation}{$\isCtx{\Gamma}{\kind}$}
\begin{mathpar}
  \infrule{Ctx-Empty}
  {}
  {\isCtx{\Empty}{\kind}}

  \infrule{Ctx-Ext}
  {\isCtx{\Gamma}{\kind}\\ \typeAgainst{T}{\kind} \\ \typec T = \Normal[+]{T}}
  {\isCtx{\Gamma, \ebind{x}{T}}{\kind}}
\end{mathpar}
\caption{Context formation}
\label{fig:ctx}
\end{figure}

==> fig-mult-alg-type-formation.tex <==
%\begin{figure}[t!]
	\declrel{Type formation (synthesis)}{$\typeSynth T \kind$}
\begin{mathpar}
  \infrule{\rulenametypeInt}{}{\typeSynth\TInt\kindtu}

  \infrule{\rulenametypeBool}{}{\typeSynth\TBool\kindtu}

  \infrule{\rulenametypeArrow}
  {\typeAgainst T\kindtl \\ \typeAgainst U\kindtl}
  {\typeSynth{\TFun TU}\kindt^\kindc{m}}

  \infrule{\rulenametypeVar}{\typec{\alpha}\colon\kind \in \Delta}{\typeSynth\alpha\kind} \\
  
  \infrule{\textcolor{red}{\rulenametypePoly}}
    {\typeSynth[\Delta,\typec{\alpha}\colon\kind] T {\kindc{\kindt^m}}}
    {\typeSynth {\forall (\typec{\alpha}\colon\kind) \typec{T}}{\kindt^\kindc{m}}}

  \infrule{\rulenametypeEnd}{}{\typeSynth\TEnd\kindsu}

  \infrule{\textcolor{red}{\rulenametypeMsgPos}}
    {\typeSynth{T}{\kind}
      % \\
      % \isSubKind\kind\kindtl \text{ or } \isSubKind\kind\kindp
    }
  {\typeSynth{{+T}}\kind}
    
  \infrule{\textcolor{red}{\rulenametypeMsgNeg}}
  {\typeSynth{T}{\kindp}}
  {\typeSynth{{-T}}\kindp}

  % \infrule{\rulenametypeDot}
  % {\typeAgainst G \kindg \\ \typeAgainst S \kindsl}
  % {\typeSynth{G.S} \kindsl}
  % 
  \infrule{\rulenametypeDotOut}
  {\typeAgainst T \kindp \\ \typeAgainst S \kindsl}
  {\typeSynth{!T.S} \kindsl}

  \infrule{\rulenametypeDotIn}
  {\typeAgainst T \kindp \\ \typeAgainst S \kindsl}
  {\typeSynth{?T.S} \kindsl}
    
  \infrule{\rulenametypePair}
  {\typeSynth{T}{\kind_1}
    \\ \typeSynth{U}{\kind_2}
    \\ \isSubKind {\kind_1, \kind_2}{\kindtl} }
  {\typeSynth{\TPair TU}{\kind_1\sqcup\kind_2}}
  
  \infrule{\rulenametypeDualS}
  {\typeSynth S \kind \\ \isSubKind\kind{\kindsl}}
  {\typeSynth{\TDual S} \kind}
  
  \infrule{\rulenametypeGuarded}
  { \typec{P : \overline\kind \to \kind \in \Delta }
    % \protocolsfull \triangleright \kind
    \\ \typeAgainst{\overline U}{\overline{\kind}}}
  {\typeSynth{P\,\overline{U}}\kind}

\end{mathpar}

  \declrel{Type formation (check-against)}{$\typeAgainst T \kind$}
  \begin{mathpar}
  % \infrule{\rulenametypeDualG}
  % {\typeAgainst G \kindg}
  % {\typeAgainst {\TDual G} \kindg}
  % 
  %   \infrule{\textcolor{red}{\rulenametypeMsg}}
  % {\typeSynth{T}{\kind} \\
  %   \isSubKind\kind\kindtl \text{ or } \isSubKind\kind\kindp}
  % {\typeAgainst{{!T}}\kindg \\ \typeAgainst{{?T}}\kindg}
  % 
  \infrule{\rulenametypeSub}
  {\typeSynth T\kind
    \\ \isSubKind \kind \kind'}
  {\typeAgainst T\kind'}
  % 
  % \infrule{\rulenametypeMsg}
  % {\typeAgainst{T}{\kindtl}}
  % {\typeAgainst{{!T}}\kindg \\ \typeAgainst{{?T}}\kindg}
  %
  % \infrule{\rulenametypeMsgP}
  % {\typeAgainst{T}{\kindpl}}
  % {\typeAgainst{{!T}}\kindg\\\typeAgainst{{?T}}\kindg
  % }
\end{mathpar}


%  \caption{Type formation rules}
%  \label{fig:type-formation}
%\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> fig-mult-alg-typing.tex <==
\declrel{Typing}{$\isExpr\Gamma eT$}
\begin{mathpar}\small
  \axiom{\rulenameexpConst}{\expSynth{\Gamma}{c}{\typeof{\termc c}}{\Gamma}}
  
  \infrule{\rulenameexpLinVar}
  {\typeSynth{T}{\kindc{v}^\lin}}
  {\expSynth{\Gamma,\termc{x}\colon\typec{T}}{x}{T}{\Gamma}}
  
  \infrule{\rulenameexpUnVar}
  {\typeSynth{T}{\kindc{v}^\un}}
  {\expSynth{\Gamma,\termc{x}\colon\typec{T}}{x}{T}{\Gamma, \termc{x}\colon\typec{T}}}
  
  \infrule{\rulenameexpLinAbs}
  {\typeAgainst{T}{\kindtl} \\ \expSynth{\Gamma_1, x\colon\typec{T}}{e}{U}{\Gamma_2}}
  {\expSynth{\Gamma_1}{\abse[\lin]xTe}{\TFun[\lin]{T}{U}}{\Gamma_2 \div \termc{x}}}

  \infrule{\rulenameexpUnAbs}
  {\typeAgainst{T}{\kindtl}
    \\ \expSynth{\Gamma_1, \termc{x}\colon\typec{T}}{e}{U}{\Gamma_2}
    \\ \Gamma_1 = \Gamma_2 \div \termc{x}}
  {\expSynth{\Gamma_1}{\abse[\un]xTe}{\TFun[\un]{T}{U}}{\Gamma_1}}
  
  \infrule{\rulenameexpTAbs}
  {\expSynth[\Delta, \typec{\alpha\colon \kind}]{\Gamma_1}{e}{T}{\Gamma_2}} 
  {\expSynth{\Gamma_1}{\tabse \alpha\kind e}{\TForall \alpha\kind T}{\Gamma_2}}

  \infrule{\rulenameexpApp}
  {\expSynth{\Gamma_1}{e_1}{\TFun{T_1}{T_2}}{\Gamma_2}
    \\\expAgainst{\Gamma_2}{e_2}{T_1}{\Gamma_3}} 
  {\expSynth{\Gamma_1}{\appe {e_1}{e_2}}{T_2}{\Gamma_3}}

  \infrule{\rulenameexpTApp}
  {\expSynth{\Gamma_1}{e}{\TForall \alpha\kind U}{\Gamma_2} \\ \typeAgainst{T}{\kind}} 
  {\expSynth{\Gamma_1}{\tappe e T}{U\tsubs{T}{\alpha}}{\Gamma_2}}

  \infrule{\rulenameexpNew}
  {\typeAgainst{T}{\kindsl}} 
  {\expSynth{\Gamma}{\newe T}{\TPair {\typec T} {\TDual T}}{\Gamma}}

  \infrule{\rulenameexpLet}
  {\expSynth{\Gamma_1}{e_1}{\TPair TU}{\Gamma_2}
    \\ \expSynth{\Gamma_2, \termc{x}\colon\typec{T}, \termc{y}\colon\typec{U}}{e_2}{V}{\Gamma_3}} 
  {\expSynth{\Gamma_1}{\lete xy{e_1}{e_2}}{V}{\Gamma_3 \div \termc{x} \div \termc{y}}}
  
  \infrule{\rulenameexpCtor}
  {\protocolsdata \triangleright \kindt^n}
  {\expSynth{\Gamma}{\constr_i}{\TForall{\overline{\alpha}}{\overline{\kindt^m}}
      {\TFun[n]{T_{i1}}{\dots \TFun[n]{T_{ik}}{\typec{D\
              \overline{\alpha}}}}}}{\Gamma}}
  
  \infrule{\rulenameexpCase1}
  {
    \expSynth\Gamma e {\typec{P\ \overline{U}}} {\Gamma_0} \\
    \protocolsdata \triangleright \kindt^n \\
    \expSynth{\Gamma_0, \termc{\overline{x_i}}\colon
      \typec{\overline{T_i\tsubs{\overline{U}}{\overline{\beta}}}}}{e_i}{V_i}{\Gamma_i}
    \\
    \typec V =_\alpha \Normal[+]{V_i}
    \\
    \Gamma' =_\alpha \Normal[+]{\Gamma_i \div \overline{x_i}}
  }
  {\expSynth{\Gamma}{\casee e {\{\constr_i\ \overline{x_i} \rightarrow
        e_i\}}}{V}{\Gamma'}}

  \infrule{\rulenameexpCase2}{
    \expSynth \Gamma e {S_0} {\Gamma_0} \\
    % \typec{S_0} \neq \typec{P\ \overline{U}} \\
    \Normal[+]{S_0} = \typec{?(\TPApp P {\overline{U}}).S} \\
    \protocolsfull \triangleright \kind \\
    \expSynth {\Gamma_0,\termc{x_i}\colon {
    \polarizedparams{?}{\overline{O_i\tsubs{\overline U}{\overline\alpha}}}{S}
    %?(\typec{\overline{T_i^\pm\tsubs{\overline G}{\overline\alpha}}.S}
    })
  } {N_i} {V_i} {\Gamma_i} \\
  \typec V = \Normal[+]{V_i} \\
  \Gamma' = \Normal[+]{\Gamma_i}
  }{
    \expSynth \Gamma {\casee e {C_i\,x_i \to N_i, \dots}} V {\Gamma'}
  }

  \infrule{\rulenameexpSelect}{
    \protocolsfull \triangleright \kind
  }{
    \expSynth \Gamma {\ESelect{C_i}}
    {\TForall{\overline{\alpha}}{\overline\kind}
      {
        {\TForall \sigma \kinds {\TFun[\un]
          {\typec{!}(\TPApp P {\overline\alpha}).\sigma}
          {\polarizedparams{!}{\overline{O_i}}{\sigma}}
%          {\overline{\blk{!}T_i^\pm}}.S
        }}}}
    \Gamma
  }

\\
  \infrule{\rulenameexpCheck}
  {\expSynth{\Gamma_1} e T {\Gamma_2} \\
    \Normal[+]T =_\alpha \Normal[+]U
  }
  {\expAgainst{\Gamma_1} e U {\Gamma_2}}
\end{mathpar}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> fig-mult-type-constants.tex <==
\declrel{Types for constants}{$\termc x\colon \typec T$}
%
\begin{align*}
  \typeof \sendk &: \TForall\alpha\kindtl{\TForall\sigma\kindsl {\alpha \to_{\un} {!\alpha}. \sigma \to_{\lin} \sigma}}
  \\
  \typeof \receivek &: \TForall\alpha\kindtl{\TForall\sigma\kindsl
                      {?\alpha. \sigma \to_{\un} \TPair\alpha\sigma}}
  \\
  \typeof \newk & : \TForall\alpha\kindsl
                  {\TFun[\un]\TUnit{\TPair\alpha{\TDual \alpha}}}
                  \\
  \typeof \forkk & : \TForall\alpha\kindt
                  {\TFun[\un]\alpha{\TUnit}}
%   \\
%   \ESelect{C_i} &: \TBForall {(\overline{\alpha\colon\kind})(\tbind\sigma\kinds)}
%                   {\oplus(\TPApp P{\overline{\alpha}}). \sigma \to  {\overline{!T_i^\pm}. \sigma}}
% &
%   \offerk &: \TBForall {(\overline{\alpha}\colon K)(\tbind\sigma\kinds)} {\&
%             (\TPApp P {\overline{\alpha}}).\sigma \to 
%   \TVariant C {{\overline{?T^\pm}}.\sigma}}
%   \\ 
%   & \text{if } \protocols
  \\ \dots
\end{align*}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> fig-mult-type-conversion.tex <==
\declrel{Type conversion}{$\isConv T T \kind$}
%
\begin{mathpar}
  \infrule{\rulenametconvReflex}{\isType T \kind}{\isConv T T \kind}

  \infrule{\rulenametconvSymm}{\isConv {T_1} {T_2} \kind}{\isConv {T_2} {T_1} \kind}

  \infrule{\rulenametconvTrans}{\isConv {T_1} {T_2} \kind \\ \isConv {T_2} {T_3} \kind}{\isConv {T_1} {T_3} \kind}

  \infrule{\rulenametconvSub}{
    \isConv {T_1}{T_2} {\kind} \\ \kind \le \kind'
  }{
    \isConv {T_1}{T_2} \kind'
  }
  \\
  \infrule{\rulenametconvDoubleS}{\isType S {\kinds^m}}{\isConv{\TDual{(\TDual S)}} S {\kinds^m}}

  % \infrule{\rulenametconvDoubleG}{\isType G \kindg}{\isConv{\TDual{(\TDual G)}} G \kindg}
  % 
  \infrule{\rulenametconvDualEnd}{}{\isConv{\TDual\TEnd}\TEnd\kindsu}
  \\
  % \infrule{\rulenametconvDualDot}{
  %   \isType G \kindg \\ \isType S {\kinds^m}
  % }{
  %   \isConv{\TDual{(G.S)}}{\TDual G . \TDual S} \kindsl
  % }
  %   
%  \infrule{}{ \isType{\forall
%      (\typec{\alpha}\colon\kindc{\kind}) \typec{T_1}}{\kindc{\kind'}} \\ \kindc{\kind'} = \kinds,\kindg }
%  { \isConv {\TDual{(\forall
%      (\typec{\alpha}\colon\kindc{\kind}) \typec{T_1} })} {\forall
%      (\typec{\alpha}\colon\kindc{\kind}) \typec{(\TDual{T_1})}}  { \kind' }}
%  
%  \\
  \infrule{\rulenametconvDualOutM}{\isType T \kindp \\ \isType S {\kindsl}}{
    \isConv{\TDual{(!T.S)}} {?T.\TDual S} \kindsl}

  \infrule{\rulenametconvDualInM}{\isType T \kindp \\ \isType S {\kindsl}}{
    \isConv{\TDual{(?T.S)}} {!T.\TDual S} \kindsl}
  % 
 %  \infrule{\rulenametconvDualOutP}{\isType T \kindp }{ \isConv{\TDual{(!T)}} {?(\TDual{T}) } \kindg}
 %  
 %  \infrule{\rulenametconvDualInP}{\isType T \kindp}{ \isConv{\TDual{(?T)}} {!(\TDual{T})} \kindg}
 %  
 %  \infrule{\rulenametconvDualProto}{
 % %  \protocols \\ 
 %  \isType{P\ \overline{T}}\kindp }{
 %  \isConv{\TDual{(P\ \overline{T}) }}{P\ \overline{T} }{\kindp} }
  \\
  \infrule{\rulenametconvNegOut}{\isType T \kindp \\ \isType S \kindsl}{\isConv {!{-T}.S}{?T.S} \kindsl}

  \infrule{\rulenametconvNegIn}{\isType T \kindp \\ \isType S \kindsl}{\isConv {?{-T}.S}{!T.S} \kindsl}
  \\
  \infrule{\rulenametconvPosOut}{\isType T \kindp \\ \isType S \kindsl}{\isConv {!{+T}.S}{!T.S} \kindsl}

  \infrule{\rulenametconvPosIn}{\isType T \kindp \\ \isType S \kindsl}{\isConv {?{+T}.S}{?T.S} \kindsl}
  \\
  \infrule{\rulenametconvPos}{\isType T \kindp}{\isConv {+T}T \kindp}

  \infrule{\rulenametconvNegInv}{\isType T \kindp}{\isConv {--T}T \kindp}
\end{mathpar}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> fig-mult-type-formation.tex <==
\begin{figure}[t!]
	\declrel{Type formation}{$\isType T\kind$}
\begin{mathpar}
  \infrule{\rulenametypeInt}{}{\isType\TInt\kindmu}

  \infrule{\rulenametypeBool}{}{\isType\TBool\kindmu}

  \infrule{{\rulenametypeArrow}}{
    \isType T \kindtl
    \\ \isType U \kindtl
  }{
    \isType{\TFun[\mult] T U}{\kindtm}}

  \infrule{\rulenametypeVar}{\typec{\alpha}\colon\kind \in \Delta}{\isType\alpha \kind}
  
  \infrule{{\rulenametypePoly}}{
    \isType[\Delta,\typec{\alpha}\colon\kind']{\typec{T}}{\kindtm}
  }{
    \isType{\forall (\typec{\alpha}\colon\kind') \typec{T}}{\kindtm}}
  
  \infrule{\rulenametypeSub}{\isType{\typec T}\kind \\ \kind \le \kind'}{\isType{\typec T}\kind'}
  \\
  \infrule{\textcolor{red}{T-Assume}}{
    \typec{P : \overline{\kind} \to \kind \in \Delta} \\
    \isType{\overline T}{\overline {\kind}}
  }{\isType{P\ \overline{T}}{\kind}}

  \infrule{\rulenametypeGuarded}{\protocolsfull \triangleright \kind \\
    \isType{\overline T}{\overline {\kind}}}{
    \isType{P\ \overline{T}}\kind}
\\
  \infrule{\rulenametypeEnd}{}{\isType\TEnd{\kindsu}}

  % \infrule{\rulenametypeDot}{\isType G \kindg \\ \isType S {\kinds^m}}{\isType{G.S} {\kindsl}}
  % 
  \infrule{\rulenametypeDualS}{\isType S {\kinds^m}}{\isType{\TDual S} {\kinds^m}}
  
  \infrule{}{\isType T \kindp \\ \isType S \kindsl}{\isType
    {! T.S}{\kindsl} \\ \isType {? T.S}{\kindsl}}
  % \\
  % \infrule{\rulenametypeMsg}{\isType{T}{\kindtl} }{
  %   \isType{{!T}}\kindg\\
  %   \isType{{?T}}\kindg
  % }
  %   
  % \infrule{\rulenametypeMsgP}{\isType{T}{\kindp}}{
  %   \isType{{\typeconstr{!}T}}\kindg\\
  %   \isType{{\typeconstr{?}T}}\kindg
  % }
  %   
  % \infrule{\rulenametypeDualG}{\isType G \kindg}{\isType {\TDual G} \kindg}
  \\
  \infrule{}{\isType T \kind} {\isType {\pneg T} \kindp}

  \infrule{}{\isType T \kind}{\isType {\ppos T} \kind}
\end{mathpar}
  \caption{Type formation}
  \label{fig:type-formation}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> fig-mult-typing.tex <==
\declrel{Typing}{$\isExpr\Gamma eT$}
%
\begin{mathpar}
  \infrule{\rulenameexpCase}{
    \protocolsfull \\
    \isExpr \Gamma M {?(\TPApp P {\overline{T}}).S} \\
    \isExpr {\Gamma,\termc{x}\colon {
    \polarizedparams{?}{\overline{O_i\tsubs{ \overline
          T}{ \overline\alpha}}^i}{S}
    %?(\typec{\overline{T_i^\pm\tsubs{\overline G}{\overline\alpha}}.S}
    })
    } {N_i} U
  }{
    \isExpr \Gamma {\casee{M}{\{C_i \,x \rightarrow N_i\}_{i\in I}}} U
  }

  \infrule{\rulenameexpSelect}{
    \protocolsfull 
  }{
    \isExpr \Gamma {\ESelect{C_i}}
    {\TBForall{(\overline{\alpha\colon\kind})}
      {
        {\TForall S \kindsl {\TFun
          {\typeconstr{!}(\TPApp P {\overline\alpha}).S}
          {\polarizedparams{!}{\overline{O_i}}{S}}
%          {\overline{\blk{!}T_i^\pm}}.S}
          }}}} 
  }\\
  \infrule{\color{red}{\rulenameexpSelect (suggestion)}}{
    \protocolk\ \typec{\proto\
    (\overline{\alpha}\colon \overline\kind)}~\blk{=}~\typec{\{\constr_i : \overline{O_i}\}_{i\in I}}
    \and (k \in I)
  }{
    \isExpr \Gamma {\ESelect{C_k}}
    {\TBForall{(\overline{\alpha\colon\kind})}
      {
        {\TForall S \kindsl {\TFun
          {\typeconstr{!}(\TPApp P {\overline\alpha}).S}
          {\polarizedparams{!}{\overline{O_i}}{S}}
%          {\overline{\blk{!}T_i^\pm}}.S}
          }}}} 
  } 
\end{mathpar}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> fig-polarized-constructors.tex <==
\begin{figure}[t!]
\declrel{Materialization and the directional operators}
{$\tosession TT = \typec{T} \quad 
  \polarizedparam - T = \typec{T} \quad
  \polarizedparam + T = \typec{T}$}
%
\begin{align*}
  \tosession {\pneg T} U &= \TIn TU & 
  \polarizedparam - {\pneg T} &= \polarizedparam + T &
  \polarizedparam + {\pneg T} &= \polarizedparam - T
  \\
  \tosession TU &= \typec{\TOut TU} & 
  \polarizedparam - T &= \pneg T &
  \polarizedparam + T &= \typec{T}
\end{align*}
In the second line $\typec T \neq \pneg U$ in all cases
\caption{Auxiliary metafunctions on session types and protocol types}
\label{fig:type-polarized-operator}
\end{figure}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> fig-type-formation.tex <==
\begin{figure}[t!]
	\declrel{Type formation}{$\hasType T\kind$}
\begin{mathpar}
  \infrule{\rulenametypeUnit}{}{\hasType\TUnit\kindt}
  
  \infrule{{\rulenametypeArrow}}{
    \hasType T \kindt
    \\ \hasType U \kindt
  }{
    \hasType{\TFun[] T U}{\kindt}}

  % \infrule{\rulenametypeInt}{}{\hasType\TInt\kindt}
  % \infrule{\rulenametypeBool}{}{\hasType\TBool\kindt}
  \infrule{\rulenametypePair}{\hasType T \kindt \\ \hasType U \kindt}{\hasType{\TPair TU}\kindt}

  \infrule{\rulenametypeVar}{\typec{\alpha}\colon\kind \in \Delta}{\hasType\alpha \kind}
  \\
  \infrule{{\rulenametypePoly}}{
    \hasType[\Delta,\typec{\alpha}\colon\kind]{\typec{T}}{\kindt}
  }{
    \hasType{\forall (\typec{\alpha}\colon\kind) \typec{T}}{\kindt}}
  
  \infrule{\rulenametypeEndW}{}{\hasType\TEndW{\kinds}}

  \infrule{\rulenametypeEndT}{}{\hasType\TEndT{\kinds}}
 
  \infrule{\rulenametypeMsg}{\hasType T \kindp \\
    \hasType S \kinds}{\hasType
    {! T.S}{\kinds} \\ \hasType {? T.S}{\kinds}}

  \infrule{\rulenametypeDualS}{\hasType S {\kinds}}{\hasType{\TDual S} {\kinds}}

  \infrule{\rulenametypeAssume}{
    \typec{\proto : \overline{\kindp} \to \kindp} \in \Delta \\
    \hasType{\overline T}{\overline {\kindp}}
  }{\hasType{\TPApp \proto {\overline{T}}}{\kindp}}
  
  \infrule{\rulenametypeMinus}{\hasType T \kindp} {\hasType {\pneg T} \kindp}
  
  \infrule{\rulenametypeSub}{\hasType{\typec T}\kind \\ \kind \le \kind'}{\hasType{\typec T}\kind'}
  % \\
  % \infrule{\rulenametypeUp}{\hasType T \kindt}{\hasType{\TUp T} \kindp}

  % \infrule{\rulenametypePlus}{\hasType T \kindp}{\hasType {\ppos T} \kindp}

  % \textcolor{red}{\infrule{\rulenametypeSemi}{
  %   \hasType T \kindp \\ \hasType U \kindp}{
  %   \hasType {T;U} \kindp
  % }}
  % \\
  % \\
  %   % \kind \in \{\kindt, \kindp\} \\
\end{mathpar}
  \caption{Type formation}
  \label{fig:type-formation}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> fig-typing.tex <==
\declrel{Typing}{$\isExpr\Gamma eT$}
%
\begin{mathpar}
  \infrule{\rulenameexpCase}{
    \protocolsfull \\
    \isExpr \Gamma M {?(\TPApp P {\overline{T}}).S} \\
    \isExpr {\Gamma,\termc{x}\colon {
    \polarizedparams{?}{\overline{O_i\tsubs{ \overline
          T}{ \overline\alpha}}^i}{S}
    %?(\typec{\overline{T_i^\pm\tsubs{\overline G}{\overline\alpha}}.S}
    })
    } {N_i} U
  }{
    \isExpr \Gamma {\casee{M}{\{C_i \,x \rightarrow N_i\}_{i\in I}}} U
  }

  \infrule{\rulenameexpSelect}{
    \protocolsfull
    \and (k \in I)
  }{
    \isExpr \Gamma {\selecte{{C_k}}}
    {\TBForall{(\overline{\alpha\colon\kind})}
      {
        {\TForall S \kinds {\TFun[]
          {\typeconstr{!}(\TPApp P {\overline\alpha}).S}
          {\polarizedparams{!}{\overline{O_k}}{S}}
%          {\overline{\blk{!}T_i^\pm}}.S}
          }}}} 
  } \\
\end{mathpar}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> introduction-old.tex <==
\section{Introduction}
\label{sec:introduction-old}

Session types
\cite{DBLP:conf/concur/Honda93,DBLP:conf/parle/TakeuchiHK94} provide a
rich type discipline for communication channels that guarantees
protocol fidelity statically. Many typing features have been
translated to the setting of session types, among them subtyping
\cite{DBLP:journals/acta/GayH05}, polymorphism
\cite{lindley17:_light_funct_session_types}, dependent types
\cite{DBLP:conf/ppdp/ToninhoCP11,DBLP:conf/fossacs/ToninhoY18,DBLP:journals/pacmpl/ThiemannV20},
and gradual types \cite{DBLP:journals/jfp/IgarashiTTVW19}. Recursive
types have been added at a very early stage
\cite{DBLP:conf/esop/HondaVK98} in a tail-recursive and equirecursive
fashion. Tail recursion was dictated by the asymmetric sequential manner of type
formation, inherited from the $\pi$-calculus. Equirecursion, where a
recursive type is considered equal to its unfoldings (or even to its
infinite unfolding), was likely chosen because unfolding should not
give rise to communication.  Moreover, there are efficient algorithms
for deciding equivalence and subtyping of recursive session types in
this form because these problems can be reduced to decision problems
on regular languages. 

However, there are protocols that cannot easily be described with
regular, tail-recursive structures. Examples are the serialization of
tree structures, stack-based protocols, non-regular protocols for
components \cite{DBLP:conf/soco/Sudholt05}, and typestate structures expressed
using fluent interfaces
\cite{DBLP:conf/ecoop/GilL16,DBLP:conf/oopsla/Xie17}.
Context-free and nested session types have been developed to  describe
these protocols
\cite{DBLP:conf/icfp/ThiemannV16,DBLP:conf/esop/Padovani17,DBLP:journals/toplas/Padovani19,DBLP:journals/corr/abs-2106-06658, DBLP:conf/esop/DasDMP21}. These
systems either equip the syntax of session types with a symmetric monoidal structure,
thus freeing them from the asymmetry of previous systems or allow
nesting of type constructors. Adding
equirecursion to such a system gives rise to context-free protocol
structures. Unfortunately, for context-free as well as nested
session types, this combination of features complicates type equivalence
significantly (doubly exponential \cite{DBLP:conf/esop/DasDMP21}) and
renders subtyping undecidable \cite{DBLP:journals/toplas/Padovani19}.

The following code example \cite{DBLP:conf/icfp/ThiemannV16} sends a
serialized binary tree using a context-free session type:
\begin{lstlisting}
data Ast = Con Int | Add Ast Ast
sendAst : Ast -> forall(s:S). mua. +{PCon: !Int, PAdd: a; a}; s -> s
sendAst t [s] c = case t of {
  Con x     -> select PCon [s] c
             |> send [Int, s] x,
  Add tl tr -> select PAdd [s] c
             |> sendAst tl [mua. +{PCon: !Int, PAdd: a; a};s]
             |> sendAst tr [s] }
\end{lstlisting}
The reading of \lstinline+data+ and \lstinline+case+ is inspired by
Haskell. The key for sending the serialized tree is the recursive session type
\lstinline_mua. +{PCon: !Int, PAdd: a; a}_. The choice operator $\oplus$
indicates a choice of sending one of the tags \lstinline+PCon+ and
\lstinline+PAdd+ and then continuing according to the session type
after the colon. For \lstinline+PCon+,
it sends the payload as determined by \lstinline+!Int+. For \lstinline+PAdd+, it recursively runs the
session type twice: \lstinline+a; a+. The semicolon operator
$\TSeq\_\_$  stands for sequential composition of session types. The operations on the
type are the usual ones: \lstinline+select+ chooses one of the tags and
sends it on the channel, \lstinline+send+ takes a number and sends it.
The operator \lstinline+|>+ is reversed function application and the
square brackets indicate type abstraction and type application.

Type checking this code in the system of \citet{DBLP:conf/icfp/ThiemannV16} is
already quite demanding. It requires unfolding of the recursion,
associativity of the $\TSeq\_\_$ operator, and distributivity of
$\TSeq\_\_$ over the choice operator. Moreover, the type checker
incorporates an expensive algorithm for type equivalence. 

A similar situation with recursive types promoted the invention of algebraic datatypes
\cite{Burstall1977a,DBLP:conf/lfp/BurstallMS80}, in a time when the decision problem
underlying type equivalence (equivalence of deterministic pushdown systems) was still open.
Algebraic datatypes combine sum-of-product types with recursion in a
way that makes type equivalence easy. In fact, the \lstinline+Ast+
datatype is isomorphic to the equirecursive type
\lstinline_mua.Int + atimesa_ where the body is a sum of product
types. Type equivalence for recursive types like this one runs into
similar difficulties with type equivalence as context-free session
types. The contribution of algebraic datatypes is the ``shrink
wrapping'' of recursion with sum-of-product types in combination with
naming the type. This combination makes type checking for algebraic datatypes
nominal and thus sidesteps all difficulties arising from recursive
types. 

The innovation of algebraic protocols consists of introducing a
shrink wrapping of recursion with choice/branch-of-sequence types combined
with naming. Compared with algebraic datatypes, we move from sum to
choice/branch and from product to sequence, which fits precisely with
the linear logic interpretation of session types \cite{DBLP:journals/mscs/CairesPT16}. 
% They implement isorecursion by reusing the
% choice tags for folding and the branch tags for driving unfolding. 
As an example, we review the serialization of binary trees using an
algebraic protocol. Like an algebraic datatype, we name the protocol,
we tag the alternatives, and we define the payload as a sequence:
\begin{lstlisting}
protocol PAst = PCon Int | PAdd PAst PAst
\end{lstlisting}
This definition only introduces two alternatives and fixes the
sequencing, but it does not indicate a direction of communication,
yet. To this end, we reuse the standard session type notation:
\begin{itemize}
\item \lstinline/!PAst/ declares sending: send a tag followed by the payload;
\item \lstinline/?PAst/ declares receiving: receive a tag, branch
  accordingly, and receive the payload.
\end{itemize}
Now we can revisit the function to send the binary tree:
\begin{lstlisting}
sendAst : Ast -> forall (s:S). !PAst.s -> s
sendAst t [s] c = case t of {
  Con x     -> select PCon [s] c
             |> send [Int, s] x,
  Add tl tr -> select PAdd [s] c
             |> sendAst tl [!PAst.s] |> sendAst tr [s] }
\end{lstlisting}
Perhaps shockingly, the code remains the same. But the types change in
several respects.
\begin{itemize}
\item The symmetric sequencing operator $\TSeq\_\_$ disappears from the syntax along with all
  problems posed by its associativity and distributivity. The
  \emph{syntax} of session types is tail-recursive as in $\TIn TS$,
  again. The context-free behavior is achieved by the typing of
  \lstinline/select PAdd/. Its type \lstinline/forall(s:S).!PAst.s -> !PAst.!PAst.s/
  ``rewrites'' a single occurrence of \lstinline/!PAst/ in front of
  the session type to two occurrences corresponding to the payload of
  the tag \lstinline/PAdd/, like a pushdown automaton operating on
  the session type.
\item Checking equivalence of algebraic protocol types is efficient:
  it is achieved by comparing their names.
\item The type \lstinline/!PAst.s/ implies that after selecting a tag,
  the payload is also sent. This mode extends to the recursive uses of
  \lstinline/PAst/ in the protocol. We would use \lstinline/?PAst.s/
  to receive a binary tree. 
\end{itemize}
This example gives a taste of the power of algebraic protocols.
In \cref{sec:algebr-sess-types} we explain how to change direction in
a protocol and how to write modular protocols by exploiting parametric
protocols.



\subsection*{Contributions}
\label{sec:contributions}

\begin{itemize}
\item Algebraic protocols (AP). We propose a new approach for defining
  recursive protocols compositionally inspired by parameterized algebraic
  datatypes. This approach combines naming, recursion, and
  choice/branch-of-sequence types analogously to algebraic
  datatypes. It adds a novel notion of direction to the payload of a
  tag. Checking type equivalence becomes simple and efficient
  (linear in the size of the types) as APs are nominal. 
\item Algebraic session types (\algst). We define a (mostly) linearly typed core calculus that
  is based on linear System~F with recursion and features session
  types based on APs. Type checking for \algst is specified  using bidirectional
  typing rules. 

  The operational semantics is presented as a labelled transition relation, adapted
  from Fowler \etal and Montesi and
  Peressotti~\cite{DBLP:conf/concur/0001KDLM21,DBLP:journals/corr/abs-2105-08996,DBLP:journals/corr/abs-2106-11818}
  for double binders and the open/close scheme for free output of the
  $\pi$-calculus~\cite{DBLP:journals/iandc/MilnerPW92b}.
  We prove type soundness via preservation and progress, where our approach offers a
  rather elegant statement (\cref{thm:progress} on \cpageref{thm:progress}). 
\item Implementation. The proposed system is fully implemented
  including several practical extensions that are documented in
  \cref{sec:implementation}. All examples in
  \cref{sec:algebr-sess-types} are checked on the implementation.
\end{itemize}

\subsection*{Overview}
\label{sec:overview}

\Cref{sec:algebr-sess-types} contains an informal introduction of
algebraic protocols with examples. \Cref{sec:types} formally
introduces kinds and types of \algst and \cref{sec:processes} defines
the statics and dynamics of expression and
processes. \Cref{sec:metatheory} presents the metatheoretical
results.
% \Cref{sec:cfst-vs-algst} gives an informal outline of
% an embedding of context-free session types to \algst.
\Cref{sec:implementation} discusses additional features of the
implementation. \Cref{sec:related,sec:conclusion} discuss related
work and conclude.

The proofs and auxiliary results are provided as supplementary material. 
The implementation is available for review in an anonymous repository
and will be submitted for artifact evaluation:
\begin{center}
  \url{https://gitlab.com/algst/algst}
\end{center}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> questions.tex <==
\section{Questions}
\label{sec:questions}

Proposition: Every nominal session typed program can be translated into a
context-free session typed program.

Conjecture: Every regular session typed program (without subtyping)
can be translated into a nominal session typed program.

This is non-trivial because regular session types
have more liberal, structural matching of recursive types. To this
end, one would have to define a normal form for recursive session
types such that type matching is decided by comparing normal
forms. The normal form can be rendered directly as a nominal type.

Conjecture: There is a context-free session-typed program that cannot
be translated to a nominal session typed program.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> type-equivalence.tex <==
\section{Deciding type equivalence}
\label{sec:type-equiv}

Type equivalence is decidable. 
\cref{fig:normalisation} contains the normalization algorithm. Its definition comprises two mutually
recursive functions $\Normal[+]{\cdot}$ and $\Normal[-]{\cdot}$. The 
superscript  is a polarity $+$ or $-$.
Function $\Normal[+]T$ is defined on all types, but 
function $\Normal[-]T$ is restricted to session types.
The negative polarity $-$ indicates that there is a pending $\TDual{\cdot}$
operation on the argument type, which is propagated by normalization.

Normalization leaves functional types unaffected. On session types,
the negative polarity is reified on type variables, it is propagated
to the session component of sending and receiving types, and each
traversal of a $\TDual\cdot$ inverts the polarity. Negative polarity also
inverts the direction of transmissions. However, the final direction is
determined by the polarity of the protocol.

\begin{example}
  Let's compute the positive normal form of
  $\TDual{(\TIn{(-\TInt)}{\alpha})}$ step by step.
  \begin{align*}
    & \Normal[+]{\TDual{(\TIn{-\TInt}{\alpha})}} \\
    ={}& \Normal[-]{{\TIn{-\TInt}{\alpha}}} \\
    ={}& \TFOut{\Normal[+]{-\TInt}}{\Normal[-]\alpha} \\
    ={}& \TFOut{\TFMinus{\Normal[+]{\TInt}}}{\TDual\alpha} \\
    ={}& \TFOut{\TFMinus{\TInt}}{\TDual\alpha} \\
    ={}& \TFOut{-{\TInt}}{\TDual\alpha} \\
    ={}& \TFIn{\TInt}{\TDual\alpha} \\
    ={}& \TIn{{\TInt}}{\TDual\alpha}
  \end{align*}
  In calculating $\Normal[-]{\typec{\TIn{-\TInt}{\alpha}}}$, the normal form of the
  protocol $\Normal[+]{-\TInt} = \typec{-\TInt}$ has negative polarity,
  which inverts the direction once more from output $\typec !$ to 
  input $\typec ?$.
\end{example}

To test whether type equivalence $\isConv TU\kind$ holds, we compute
the normal forms $\Normal[+]T$ and $\Normal[-]U$ and compare them
modulo $\alpha$ convertibility. 
We write $\typec T =_\alpha \typec U$ if types $\typec T$ and $\typec U$ are
$\alpha$-equivalent. The following propositions establish soundness and
completeness of this algorithm.

Every type is convertible to its normal form.
\begin{proposition}[Kind preservation]~\label{lemma:kind-preservation}
  \begin{enumerate}
  \item For all $\typeSynth T\kind$,  $\isConv{\Normal[+] T}T\kind$.
  \item For all $\typeSynth T\kinds$,  $\isConv{\Normal[-] T}{\TDual T}\kinds$.
  \end{enumerate}
\end{proposition}
\begin{proof}
  See Agda development \texttt{nf-sound+} and \texttt{nf-sound-}.
\end{proof}

\begin{corollary}[Soundness] Let $\typeSynth T\kind$ and $\typeSynth U\kind$.
  \begin{enumerate}
  \item If $\Normal[+] T =_\alpha \Normal[+] U$, 
    then $\isConv TU\kind$.
  \item If $\kind = \kinds$ and  $\Normal[-] T =_\alpha \Normal[-]
    U$, then $\isConv TU\kinds$.
  \end{enumerate}
\end{corollary}
\begin{proof}
  Item~1. Suppose that $\Normal[+] T =_\alpha \Normal[+] U$. By
  Lemma~\ref{lemma:kind-preservation}, we have  $\isConv{\Normal[+]
    T}T\kind$ and  $\isConv{\Normal[+] U}U\kind$. Conclude by symmetry
  and transitivity of conversion as ${=_\alpha} \subseteq {\equiv}$.

  The proof for item~2 is analogous.
\end{proof}

If two types are convertible, then their normal forms are equal.
\begin{proposition}[Completeness]   Let $\isConv TU\kind$. 
  \begin{enumerate}
  \item  $\Normal[+]T =_\alpha \Normal[+]U$.
  \item    If $\kind=\kinds$, then $\Normal[-]T =_\alpha \Normal[-]U$. 
  \end{enumerate}
\end{proposition}
\begin{proof}
  See Agda development \texttt{nf-complete} and \texttt{nf-complete-}.
\end{proof}

To obtain a complexity bound for the computation of a normal form, we
characterize the output of the function $\Normal T$, that is, the
syntax of normal forms. 
Normal forms for well formed types are $\typec{R^-}$ such that:
%
\begin{align*}
  \typec R^- \grmeq\;& \typec{R} \grmor \pneg{R}
  \\
  \typec{R} \grmeq\;&
  % functional types
  \TUnit \grmor \TFun[]{R}{R} \grmor \TPair{R}{R} \grmor
  \typec{\alpha} \grmor \TForall \alpha \kind {R}
  % session types
  \grmor \TEndW \grmor \TEndT \grmor \TIn{R}{R} \grmor \TOut{R}{R} \grmor \TDual{\alpha}
  % protocol and data types
  \grmor \TPApp X {\overline{R^-}}
\end{align*}
Essentially, the negative polarity can only occur at most once at the top level (of
a type of kind $\kindp$) and in the parameters of a protocol type. The
$\TDual\cdot$ operator only appears on type variables.
\begin{lemma}\label{lemma:syntax-of-type-normal-forms}
  If $\Normal[\pm]T = \typec{T'}$, then $\typec{T'}$ is described by $\typec{R^-}$.
\end{lemma}
\begin{proof}
  See Agda development \texttt{nf-normal}.
\end{proof}
\begin{proposition}
  For each $\typeSynth T\kind$, 
  the run time of $\Normal[\pm]T$ is in $O(|\typec{T}|)$.
\end{proposition}
\begin{proof}
  A run of $\Normal T$ visits each of the $|\typec{T}|$ nodes in
  the input type once. At each node, it either reconstructs the type
  from the normal forms of the sub-types in $O(1)$ time, or (in the transmission rules) it applies polarity
  correction to normal forms. By
  Lemma~\ref{lemma:syntax-of-type-normal-forms}, a normal form  
  starts with at most one negative polarity, so  correction
  takes at most two steps, that is $O(1)$. 
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

